A Broad Study on the Transferability of Visual Representations with Contrastive Learning

Tremendous progress has been made in visual representation learning, notably with the recent success of self-supervised contrastive learning methods. Supervised contrastive learning has also been shown to outperform its cross-entropy counterparts by leveraging labels for choosing where to contrast. However, there has been little work to explore the transfer capability of contrastive learning to a different domain. In this paper, we conduct a comprehensive study on the transferability of learned representations of different contrastive approaches for linear evaluation, full-network transfer, and few-shot recognition on 12 downstream datasets from different domains, and object detection tasks on MSCOCO and VOC0712. The results show that the contrastive approaches learn representations that are easily transferable to a different downstream task. We further observe that the joint objective of self-supervised contrastive loss with cross-entropy/supervised-contrastive loss leads to better transferability of these models over their supervised counterparts. Our analysis reveals that the representations learned from the contrastive approaches contain more low/mid-level semantics than cross-entropy models, which enables them to quickly adapt to a new task. Our codes and models will be publicly available to facilitate future research on transferability of visual representations.

==> ICCV2021/Main/6_extra.tex <==
% \subsection{Transferability of contrastive learning in Video Action Recognition}
% In this section, we explore the effectiveness of the studied methods in transfer learning for a video action recognition task. We use the Resnet-(2+1)D backbone~\cite{tran2018closerr2plus1}, train the networks on the Kinetics400 training set \cite{carreira2017quokinetics}, and perform fixed feature linear evaluation on the UCF101 \cite{soomro2012ucf101}, HMDB51 \cite{kuehne2011hmdb}, ARID \cite{xu2020arid}, and Diving48 \cite{li2018resounddiving48} datasets. More details about the parameter settings for training and evaluation are provided in the supplementary. Table \ref{tab:video_linear} reports the transfer accuracy of different methods on the downstream video datasets. We find that \CEplusMOCO and \MIT perform slightly better than \CE; however, \MOCO and \MITplusMOCO perform worse than \CE in all datasets. As action recognition is much different than image classification task because of temporal dependency in videos, it is possible that utilizing other modalities might improve representation quality of contrastive models in video domain.   

% \begin{table}[ht!]
%     \centering
%     \begin{adjustbox}{max width=\linewidth}
%     \InputTable{linear_3d_bn}
%     \end{adjustbox}
%     \caption{Performance of different Kinetics400 pretrained models on the downstream video action recognition dataset. We use the pretrained backbones as fixed feature extractors and train a linear layer to adapt to the downstream video domain.}
%     \label{tab:video_linear}
% \end{table}



==> ICCV2021/Tables/R_layer-2.tex <==
\begin{tabular}{ll}
\toprule
{} & Intra-class distance \\
\midrule
ce       &         0.79 $\pm$ 0.03 \\
ce+moco  &         0.79 $\pm$ 0.03 \\
mit      &         0.79 $\pm$ 0.03 \\
mit+moco &         0.79 $\pm$ 0.03 \\
moco     &         0.80 $\pm$ 0.03 \\
\bottomrule
\end{tabular}


==> ICCV2021/Tables/R_layer-3.tex <==
\begin{tabular}{ll}
\toprule
{} & Intra-class distance \\
\midrule
ce       &         0.79 $\pm$ 0.02 \\
ce+moco  &         0.78 $\pm$ 0.03 \\
mit      &         0.77 $\pm$ 0.03 \\
mit+moco &         0.78 $\pm$ 0.02 \\
moco     &         0.79 $\pm$ 0.03 \\
\bottomrule
\end{tabular}


==> ICCV2021/Tables/R_layer-4.tex <==
\begin{tabular}{ll}
\toprule
{} & Intra-class distance \\
\midrule
ce       &         0.78 $\pm$ 0.02 \\
ce+moco  &         0.75 $\pm$ 0.03 \\
mit      &         0.77 $\pm$ 0.02 \\
mit+moco &         0.78 $\pm$ 0.02 \\
moco     &         0.78 $\pm$ 0.02 \\
\bottomrule
\end{tabular}


==> ICCV2021/Tables/header.tex <==
{} &  \rot{ChestX} &  \rot{CropDisease} &  \rot{DTD} &  \rot{DeepWeeds} &  \rot{EuroSAT} &  \rot{Flowers102} &  \rot{ISIC} &  \rot{Kaokore} &  \rot{Omniglot} &  \rot{Resisc45} &  \rot{SVHN} &  \rot{Sketch} &  \rot{Mean} \\

==> ICCV2021/Tables/imagenet_c.tex <==
\begin{tabular}{l|c}
\toprule
    Method & mCE  \\
\midrule
    \CE &  60.79 \\
    \MOCO & 68.87 \\
    % CUHK & 65.07 & \\
    \MIT & 54.23  \\
    \CEplusMOCO & 54.27  \\
    \MITplusMOCO & 54.39  \\
\bottomrule
\end{tabular}

==> ICCV2021/Tables/imagenet_eval_ce_strong.tex <==
\begin{tabular}{l|c c c| c c}
\toprule
           & \multicolumn{3}{c|}{ImageNet} & \multicolumn{2}{c}{Stylized ImageNet} \\
    Method & Top-1(\%) & NLL & ECE(\%) & Top-1(\%) & ECE(\%) \\
\midrule
    \CE &  76.60 & 0.9575 & 6.63 & 7.50 & 33.19 \\
    \CEstrong &  76.80 & 0.9774 & 6.45 & 9.87 & 26.47 \\
\bottomrule
\end{tabular}


==> ICCV2021/Tables/sin.tex <==
\begin{tabular}{l|c c}
\toprule
    Method & Top-1 & ECE  \\
\midrule
    \CE &  6.52 & 29.38 \\
    \MOCO &  5.34 & 21.59 \\
    % CUHK & 65.07 & \\
    \MIT & 10.12 & 16.35 \\
    \CEplusMOCO & 9.77 & 24.36  \\
    \MITplusMOCO & 9.70 & 13.42  \\
\bottomrule
\end{tabular}
